Integrating Multi-scale Contextualized Information for Byte-based Neural Machine Translation

Subword tokenization is a common method for vocabulary building in Neural Machine Translation (NMT) models. However, increasingly complex tasks have revealed its disadvantages. First, a vocabulary cannot be modified once it is learned, making it hard to adapt to new words. Second, in multilingual translation, the imbalance in data volumes across different languages spreads to the vocabulary, exacerbating translations involving low-resource languages. While byte-based tokenization addresses these issues, byte-based models struggle with the low information density inherent in UTF-8 byte sequences. Previous works enhance token semantics through local contextualization but fail to select an appropriate contextualizing scope based on the input. Consequently, we propose the Multi-Scale Contextualization (MSC) method, which learns contextualized information of varying scales across different hidden state dimensions. It then leverages the attention module to dynamically integrate the multi-scale contextualized information. Experiments show that MSC significantly outperforms subword-based and other byte-based methods in both multilingual and out-of-domain scenarios. Code can be found in https://github.com/ictnlp/Multiscale-Contextualization.

==> tables/opus7.tex <==
\begin{table*}[h]
\centering
\scalebox{0.67}{
\begin{tabular}{l|c|ccccccc|ccccccc|c}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Appraoch}} & \multirow{2}{*}{Param.} & \multicolumn{7}{c|}{XX$\rightarrow$En}                                                                                                                                                                                                                                         & \multicolumn{7}{c|}{En$\rightarrow$XX}                                                                                                                                                                                                                                          & \multirow{2}{*}{AVG.}              \\ \cline{3-16}
\multicolumn{1}{c|}{}                          &                         & Ar                                 & De                                 & Fr                                 & Nl                                 & Ru                                  & Zh                                 & AVG.                                & Ar                                 & De                                 & Fr                                 & Nl                                 & Ru                                  & Zh                                  & AVG.                                &                                    \\ \hline
Single-Trans.                                  & 44.6M                   & \multicolumn{1}{l}{\textbf{32.94}} & \multicolumn{1}{l}{\textbf{31.20}} & \multicolumn{1}{l}{\textbf{30.53}} & \multicolumn{1}{l}{\textbf{28.49}} & \multicolumn{1}{l}{\textbf{29.94*}} & \multicolumn{1}{l}{\textbf{32.00}} & \multicolumn{1}{l|}{\textbf{30.85}} & \multicolumn{1}{l}{\textbf{16.86}} & \multicolumn{1}{l}{\textbf{28.29}} & \multicolumn{1}{l}{\textbf{27.71}} & \multicolumn{1}{l}{\textbf{26.71}} & \multicolumn{1}{l}{\textbf{20.41*}} & \multicolumn{1}{l}{\textbf{30.18*}} & \multicolumn{1}{l|}{\textbf{25.03}} & \multicolumn{1}{l}{\textbf{27.94}} \\ \hline
Multi-Trans.                                   & 44.6M                   & 26.87                              & 28.58                              & 26.50                              & 25.45                              & 26.10                               & 25.99                              & 26.58                               & 12.77                              & 25.49                              & 23.81                              & 22.69                              & 16.99                               & 25.06                               & 21.14                               & 23.86                              \\ \hline
Byte-\textit{n}CF                                       & 47.0M                   & 29.05                              & 29.51                              & 27.99                              & 26.56                              & 27.85                               & \textbf{28.92}                     & 28.31                               & 13.68                               & 26.47                              & \textbf{25.29}                              & 24.12                               & 18.59                               & 26.88                                & 22.51                                & 25.48                              \\ \hline
MSC                                            & 44.8M                   & \textbf{29.57}                     & \textbf{29.81}                     & \textbf{28.02}                     & \textbf{26.92}                     & \textbf{28.05}                      & 28.35                              & \textbf{28.45}                      & \textbf{13.79}                     & \textbf{26.95}                     & 25.23                     & \textbf{24.53}                     & \textbf{19.05}                      & \textbf{27.12}                      & \textbf{22.78}                      & \textbf{25.62}                     \\ \hline
\end{tabular}
}
\caption{The experiment results on OPUS7 dataset. "Single-Trans." means training one model for each of the 12 translation directions, which are treated as the upper-bound. The "$*$" sign indicates that the training is unstable and was failed at the first time. All the other approaches are trained on the 12 directions together.}
\label{table:opus7}
\end{table*}
